Calibration: A Simple Trick for Wide-table Delta Analytics

Data analytics over normalized databases typically requires computing and materializing expensive joins (wide-tables). Factorized query execution models execution as message passing between relations in the join graph and pushes aggregations through joins to reduce intermediate result sizes. Although this accelerates query execution, it only optimizes a single wide-table query. In contrast, wide-table analytics is usually interactive and users want to apply delta to the initial query structure. For instance, users want to slice, dice and drill-down dimensions, update part of the tables and join with new tables for enrichment. Such Wide-table Delta Analytics offers novel work-sharing opportunities. This work shows that carefully materializing messages during query execution can accelerate Wide-table Delta Analytics by >10^5x as compared to factorized execution, and only incurs a constant factor overhead. The key challenge is that messages are sensitive to the message passing ordering. To address this challenge, we borrow the concept of calibration in probabilistic graphical models to materialize sufficient messages to support any ordering. We manifest these ideas in the novel Calibrated Junction Hypertree (CJT) data structure, which is fast to build, aggressively re-uses messages to accelerate future queries, and is incrementally maintainable under updates. We further show how CJTs benefit applications such as OLAP, query explanation, streaming data, and data augmentation for ML. Our experiments evaluate three versions of the CJT that run in a single-threaded custom engine, on cloud DBs, and in Pandas, and show 30x - 10^5x improvements over state-of-the-art factorized execution algorithms on the above applications.

==> content/design.tex <==
\section{Design and Optimizations (Deleted)}
\label{designsec}

In this section, we illustrate the trade-offs between different designs of Junction Hypertree, and discuss further optimizations.

\subsection{Junction Hypertree Design}
We start with the discussion of how to find the Junction Hypertree given relations. Then, we discuss how to design Junction Hypertree given potential workloads.


\stitle{Find Junction Hypertree.}
We discuss how to build Junction Hypertree given a set of relations $\textbf{R} = \{R_1, R_2 ... , R_n\}$. As discussed in section 4, finding the Junction Hypertree with minimum fractional hypertree width is NP-hard~\cite{fischl2018general}. However, most of databases have simple schema and are usually acyclic. For acyclic join graph, we commonly create Junction Hypertree where each bag contains one relation, and this Junction Hypertree has minimum fractional hypertree width.

For more complex databases with galaxy schema, we need to eliminate cycle by clutering relations into one bag. This is similar to building Junction Tree for undirected graph, and greedy algorithm has been widely used in Probabilistic Grpahical Model \cite{geiger2003optimizing} to search for small Junction Tree over graphical models with great performance over real-world datasets \cite{kask2011pushing}. (cite our paper of greedy algorithm)

\subsection{Optimization}

We introduce lazy calibration and other optimizations opportunities in Calibrated Junction Hypertree.



==> content/fmp.tex <==
\begin{figure}[b]
  \centering
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/bayesian_network.pdf}
         \caption{Bayesian Network.}
         \label{fig:bayesian}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.18\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/joint_distribution.pdf}
         \caption{Joint Distribution.}
         \label{fig:joint}
     \end{subfigure}
     \hfill
    \begin{subfigure}[b]{0.25\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/pgm_msg.pdf}
         \caption{Message passing.}
         \label{fig:pgmmsg}
     \end{subfigure}
     \hfill
  \caption{Message Passing}
%   \label{fig:buildDtree}
\end{figure}




==> content/tcomplexity.tex <==

\begin{table*}[h!]
\begin{center}
\setlength{\tabcolsep}{0.2em} % for the horizontal padding
\begin{tabular}{ | m{6em} | m{40em}|} 
\hline
Complexity & Works \\
\hline
\texttt{fec}~\cite{atserias2008size} & 
Data Cube~\cite{gray1997data}, Traditional ML~\cite{ghoting2011systemml,hellerstein2012madlib}, 
Explanation Ready Database~\cite{roy2015explaining},
First-order IVM~\cite{zhuge1995view}
\\ 
\hline
\texttt{fhtw}~\cite{gottlob2009generalized} &
Factorised Representation~\cite{olteanu2015size} ,
Factorised ML~\cite{schleich2016learning,schleich2019layered},
Semiring Aggregation~\cite{abo2016faq,joglekar2015aggregations,green2007provenance},\newline
Factorised IVM~\cite{nikolic2018incremental,idris2017dynamic},
Higher-order IVM~\cite{ahmad2012dbtoaster}, Build \cjt 
 \\
\hline
$\texttt{fhstw}_\phi$ & Query over \cjt $\phi$\\
\hline
\end{tabular}

\end{center}
\caption{Comparison of complexity classes between different works.}
\label{table:complexity}
\end{table*}

